Multiple inflation and the WMAP 'glitches' II. Data analysis and cosmological parameter extraction

Detailed analyses of the WMAP data indicate possible oscillatory features in the primordial curvature perturbation, which moreover appears to be suppressed beyond the present Hubble radius. Such deviations from the usual inflationary expectation of an approximately Harrison-Zeldovich spectrum are expected in the supergravity-based 'multiple inflation' model wherein phase transitions during inflation induce sudden changes in the mass of the inflaton, thus interrupting its slow-roll. In a previous paper we calculated the resulting curvature perturbation and showed how the oscillations arise. Here we perform a Markov Chain Monte Carlo fitting exercise using the 3-year WMAP data to determine how the fitted cosmological parameters vary when such a primordial spectrum is used as an input, rather than the usually assumed power-law spectrum. The 'concordance' LCDM model is still a good fit when there is just a 'step' in the spectrum. However if there is a 'bump' in the spectrum (due e.g. to two phase transitions in rapid succession), the precision CMB data can be well-fitted by a flat Einstein-de Sitter cosmology without dark energy. This however requires the Hubble constant to be h ~ 0.44 which is lower than the locally measured value. To fit the SDSS data on the power spectrum of galaxy clustering requires a ~10% component of hot dark matter, as would naturally be provided by 3 species of neutrinos of mass ~0.5 eV. This CHDM model cannot however fit the position of the baryon acoustic peak in the LRG redshift two-point correlation function. It may be possible to overcome these difficulties in an inhomogeneous Lemaitre-Tolman-Bondi cosmological model with a local void, which can potentially also account for the SN Ia Hubble diagram without invoking cosmic acceleration.

==> stepdegen.tex <==
\subsection{$\Lambda$CDM `step' model degeneracies}
 
The results indicate a strong parameter degeneracy amongst the models
with one phase transition. Moving in parameter space along the direction of
the degeneracy, $\Delta m^2$ increases, while $\mathcal{P_R}^{(0)}$ and 
$k_1$ both decrease.

\begin{figure}[tbh]
\includegraphics[angle=-90,scale=0.5]{all1degen1.eps}
\caption{\label{all1degen1} 
The degeneracy between the large-scale amplitude of the primordial
 spectrum and the fractional change in the inflaton mass according to
 eq.(\ref{degen1}), with the `data' points taken from
 Table~\ref{tab:all1step}.}
\end{figure}  

The degeneracy arises because the amplitude of the TT spectrum on the
scale of the acoustic peaks is governed by the combination
$\mathcal{P_R}^{(1)}\mathrm{e}^{-2\tau}$, where $\mathcal{P_R}^{(1)}$
is the amplitude of the primordial spectrum on small scales. In
the slow-roll approximation the latter is given by
\begin{equation}
P_{\mathcal{R}}^{(1)} = 
\frac{P_{\mathcal{R}}^{(0)}}{\left(1 - \Delta m^2\right)^2}.
\label{degen1}
\end{equation}
The {\sl WMAP} data tightly constrains the value of
$\mathcal{P}_{\mathcal{R}}^{(1)}\mathrm{e}^{-2\tau}$, and so $\tau$
and $\mathcal{P_R}^{(1)}$ are positively correlated, with
$\mathcal{P_R}^{(1)} \propto \mathrm{e}^{2\tau}$. As a result $\tau$
at fixed $\Delta m^2$ is positively correlated with $\mathcal{P_R}^{(0)}$. 
This reflects the well-known degeneracy between the optical depth and 
the normalisation of the TT spectrum. For $n=15$ to $n=17$ increasing 
$\Delta m^2$ raises the amplitude of the TT spectrum for low multipoles 
due to the increased height of the first peak in $\mathcal{P_R}(k)$. Thus 
$\tau$ falls going from $n=15$ to $n=17$ because decreasing $\tau$ reduces 
the amplitude of the TT spectrum on large scales relative to small scales.

 
The value of $\mathcal{P_R}^{(1)}$ is 
constrained after marginalising over $\tau$, which means that the
relationship between $\Delta m^2$ and
$\mathcal{P_R}^{(0)}$ is fitted well by
\begin{equation}
P_{\mathcal{R}}^{(0)} = P_{\mathcal{R}}^{\rm HZ}\left(1 - \Delta m^2\right)^2,
\label{prm}
\end{equation}
where $P_{\mathcal{R}}^{\rm HZ}$ is a constant (being the amplitude of
a scale-invariant Harrison-Zeldovich primordial spectrum). This is 
illustrated in Fig.\ref{all1degen1} using results from Table~\ref{tab:all1step}.

The parameter $k_1$ is negatively correlated with $\Delta m^2$ because
the higher cosmic variance at low $\ell$ allows the data to
accommodate more prominent features in the primordial spectrum at
smaller $k$. The likelihood distributions of $k_1$ are strongly
non-Gaussian, as shown in Fig.\ref{all1Lmany2a}. Each distribution has
maxima wherever the oscillations in the corresponding TT spectrum due
to the phase transition match the glitches in the {\sl WMAP}
measurements.
